Neural Network Acceleration of Iterative Methods for Nonlinear Schr\"odinger Eigenvalue Problems

We present a novel approach to accelerate iterative methods to solve nonlinear Schr\"odinger eigenvalue problems using neural networks. Nonlinear eigenvector problems are fundamental in quantum mechanics and other fields, yet conventional solvers often suffer from slow convergence in extreme parameter regimes, as exemplified by the rotating Bose- Einstein condensate (BEC) problem. Our method uses a neural network to predict and refine solution trajectories, leveraging knowledge from previous simulations to improve convergence speed and accuracy. Numerical experiments demonstrate significant speed-up over classical solvers, highlighting both the strengths and limitations of the approach.

==> figs/commands.tex <==
\newcommand\meanRiter{368.57}
\newcommand\medianRiter{40.00}
\newcommand\meanEiter{289.45}
\newcommand\medianEiter{98.50}
\newcommand\meanRpercIter{7.19}
\newcommand\medianRpercIter{6.56}
\newcommand\meanEpercIter{10.19}
\newcommand\medianEpercIter{15.62}
\newcommand\meanRrhos{-881.15}
\newcommand\medianRrhos{-20.97}
\newcommand\meanErhos{-17.25}
\newcommand\medianErhos{48.01}


==> figs/figure_hist_its.tex <==
\begin{figure}
\centering
\begin{subfigure}{.5\textwidth}
  \centering
    \captionsetup{width=.9\textwidth}
  \input{./figs/histograms/hist_its.tex}
  \label{fig:sub1}
    \subcaption{Number of iterations saved by neural network enhancement of the algorithm when neural network was applied at a randomly chosen iteration. 
    Improvement was achieved in 82.4\% of cases.
    }
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \captionsetup{width=.9\textwidth}
  \input{./figs/histograms/hist_its_enhanced.tex}  
  \label{fig:sub2}
  \subcaption{Number of iterations saved by neural network enhancement of the algorithm when neural network was applied via the previously described acceleration strategy.
  Improvement was achieved in 91.8\% of cases.
  }
\end{subfigure}
    \caption{Histograms of the number of iterations saved by the neural network-accelerated algorithms, evaluated on all 500 test cases. 
    In blue are the cases, where the enhanced and classical algorithm converged to the same local minimum, in orange the cases of different minima. 
    The dashed bars denote the cases falling outside the interval [-1000,1000].
    }
\label{fig:figure_hist_its}
\end{figure}
    
